Design and Control of a Micro Overactuated Aerial Robot with an Origami Delta Manipulator

This work presents the mechanical design and control of a novel small-size and lightweight Micro Aerial Vehicle (MAV) for aerial manipulation. To our knowledge, with a total take-off mass of only 2.0 kg, the proposed system is the most lightweight Aerial Manipulator (AM) that has 8-DOF independently controllable: 5 for the aerial platform and 3 for the articulated arm. We designed the robot to be fully-actuated in the body forward direction. This allows independent pitching and instantaneous force generation, improving the platform's performance during physical interaction. The robotic arm is an origami delta manipulator driven by three servomotors, enabling active motion compensation at the end-effector. Its composite multimaterial links help reduce the weight, while their flexibility allow for compliant aerial interaction with the environment. In particular, the arm's stiffness can be changed according to its configuration. We provide an in depth discussion of the system design and characterize the stiffness of the delta arm. A control architecture to deal with the platform's overactuation while exploiting the delta arm is presented. Its capabilities are experimentally illustrated both in free flight and physical interaction, highlighting advantages and disadvantages of the origami's folding mechanism.

==> delta_kin_backup.tex <==

The kinematic relation for a generic leg $i=\{1,2,3\}$ is
\begin{equation}
    \Pv_{h,i} + \lv_{p,i} + \lv_{d,i} = \eefPose + \Pv_{a,i} ,
\end{equation}
with $\Pv_{h,i} = \left[ 0 \vSpace r_D \vSpace 0 \right]\transpose$, $\lv_{p,i} = \left[ 0 \vSpace l_p\cos{\deltaJoint} \vSpace l_p \sin{\deltaJoint} \right]\transpose$ and $\Pv_{a,i} = \left[ 0 \vSpace r_E \vSpace 0 \right]\transpose$.
% \begin{equation}
%     \D \Pv_{h,i} =
%     \begin{bmatrix}
%         0 \\
%         r_D \\
%         0
%     \end{bmatrix};\quad \D \lv_{p,i} = 
%     \begin{bmatrix}
%         0 \\
%         l_p \cos{\theta_i} \\
%         l_p \sin{\theta_i}
%     \end{bmatrix}
% \end{equation}
We then compute the true length of the distal link as
\begin{equation}
    \lv_{d,i}(\D\eefPose) = 
    \D\eefPose - 
    \begin{bmatrix}
        0 \\
        l_p \cos{\deltaJoint} + r_D - r_E \\
        l_p \sin{\deltaJoint}
    \end{bmatrix}
    % a = r_D - r_E
\end{equation}

% \begin{equation}
%     \label{ankle_transform}
%     \D \Pv_{a,i} =
%     \begin{bmatrix}
%         0 \\
%         r_E \\
%         0 \\
%     \end{bmatrix}
% \end{equation}

%where in \eqref{ankle_transform} we make use of the constraint that the end effector platform of a delta robot always remains parallel to the base and is only allowed translational motion.
To solve for the variable $\theta_1$ the constraint on the distal leg length is used:
\begin{equation}
    \label{quadratic_equation}
    l_{d,i} = \norm{\D \lv_{d,i}} = 
    \norm{\D \Pv_{E} + \D \Pv_{a,i} - \D \Pv_{h,i} - \D \lv_{p,i}},
\end{equation}
with the origami distal leg expression
\begin{equation}
    l_{d,i} = \sqrt{\D p_{E,x}^2 + \left(\sqrt{l_m^2 - \D p_{E,x}^2} + 2l_e\right)^2}
\end{equation}
By squaring both sides of \eqref{quadratic_equation} we finally get the equation:
\begin{equation}
    \label{squared_leg_contraint_equation}
    E_1 \cos{\theta_1} + F_1 \sin{\theta_1} + G_1 = 0,
\end{equation}
where
\begin{subequations}
    \begin{IEEEeqnarray} {ll}
        E_1 = 2 l_p (\D p_{E,y} + a) \\
        F_1 = 2\D p_{E,z} l_p \\
        \begin{split}
            G_1 = \D p_{E,x}^2 + \D p_{E,y}^2 + \D p_{E,z}^2 + a^2 \\
            + l_p^2 + 2 \D p_{E,y} a - l_{d,i}^2
        \end{split}
    \end{IEEEeqnarray}
\end{subequations}

$\theta_1$ is finally solved for by applying the tangent half-angle substitution and converting \eqref{squared_leg_contraint_equation} to a quadratic equation:
%\begin{equation}
%        t_i \coloneqq \tan{\frac{\theta_i}{2}} \quad
%        \cos{\theta_i} = \frac{1 - t_i^2}{1 + t_i^2} \quad
%        \sin{\theta_i} = \frac{2t_i}{1 + t_i^2}
%\end{equation}

%\begin{equation}
%    (G_i - E_i)t_i^2 + (2F_i)t_i + (G_i + E_i) = 0
%\end{equation}

\begin{equation}
    t_{i_{1,2}} = \frac{-F_i \pm \sqrt{E_i^2 + F_i^2 - G_i^2}}{G_i - E_i}
\end{equation}

\begin{equation}
    \theta_i = 2 \tan^{-1}(t_i^+)
\end{equation}

The same derivation holds for the solution of the other two manipulator legs that are each rotated by 120°.

==> platform_controller.tex <==
\subsection{Aerial platform}
\begin{itemize}
    \item Pose controller.\\
        %   \begin{figure*}
        %       \centering              \includegraphics[width=1\textwidth]{Diagram_mini_voliro_code.png}
        %       \caption{Diagram for pose control on Mini Voliro}
        %       \label{pics:diagram}
        %   \end{figure*}
          %\Elia{
          %    How do we formally define the control errors and the control action? Consider a fixed world frame $\frameW$ and a body frame $\frameB$ attached to the drone's body in its \ac{COM}.
          %    We then define the rotation matrix body to world frame as $\rotMatWB \in \nR{3 \times 3}$ and the position of the body frame's origin in the world frame as $\W{\pos} \in \nR{3}$. Consider also a reference trajectory $\rotMatWB\refer$ and $\W{\pos}\refer$}
          Consider a fixed world frame $\frameW$, a body frame $\frameB$ attached to the drone's body in its \ac{COM} and a frame $\frameL$ which has the same origin and $y$ axis of the $\frameB$, but its pitch angle with respect to frame $\frameW$ will always be $0$.
          %
          This frame is necessary to decouple the fully actuated pitching dynamics from the underactuated rolling dynamics of conventional \acp{MAV}.
          %
          For instance, a forward position command along the $x_L$ axis would be transformed in a command along $x_B$ and $z_B$ axes in the $\frameB$ frame.
          %in this case for example a forward desired movement will be executed with a displacement in the x-direction only as it is in the L frame, while in the body frame the forward movement with a pitch angle would result in a displacement in both x and z-directions depending on the pitch angle.
            %
            We then define the rotation matrix from $\frameW$ to $\frameL$ as $\rotMatLW \in \nR{3 \times 3}$ and the position of the body frame's origin in the world frame as $\W\pos \in \nR{3}$.
            %
            We then define as $\W(\cdot)$ and $\L(\cdot)$ quantities defined in the $\frameW$ and $\frameL$ frames, respectively.
          %
            Position control errors are first computed in the $\frameL$ frame as
            \begin{equation} \label{eq3}
            \begin{split}
            \positionErrorL &=  \rotMatLW (\W\pos\refer - \W\pos),\\
            \velocityRefL &= \kpPos \positionErrorL  +  \kiPos \int_0^t\positionErrorL ,\\
            \velocityErrorL &= \velocityRefL%\rotMatLW\velocityRefW
            - \L\vel ,\\
            \linearCumulativeErrorL &= \kpVel \velocityErrorL + \kiVel \int_0^t\velocityErrorL -\kdVel \acc,\\
            %\linearAccelerationL &= \linearCumulativeErrorL + R_{LW} \setpointAccelerationW, \\
            %\linearAccelerationL &-= R_{LW} \gravityW, \\
            \B\forceCommand &= \rotMatLB\transpose \mass \linearCumulativeErrorL + \rotMatWB\transpose \gravityForce ,
            \end{split}
            \end{equation}
            %
            where $\positionErrorL \in \nR{3}$ is the position error, $\W\pos\refer \in \nR{3}$ the position reference, $\W\pos \in \nR{3}$ the position in world frame, $\velocityRefW \in \nR{3}$ the velocity reference, $\velocityErrorL \in \nR{3}$ the velocity error, $\L\vel \in \nR{3}$ the platform's velocity, $\linearCumulativeErrorL\in\nR{3}$ the total linear error given by the combination of velocity and position errors and $\kpPos$, $\kiPos$, $\kpVel$, $\kiVel$, $\kdVel \in \nR{3 \times 3}$ are positive definite and diagonal gain matrices. $\B\forceCommand \in \nR{3}$ is the linear force command,
            %$\setpointAccelerationW \in \nR{3}$ is the acceleration reference in world frame which consider the input given to the drone. 
            $\gravityForce \in \nR{3}$ is the gravity force vector, and $m \in \nR{}$ is the mass of the MAV.
            %
            The linear error in L frame is used to calculate the desired linear acceleration also in L frame, then after subtracting gravity the desired force vector in L frame can be calculated. \\
            %
            The L frame vector force is converted into body frame to provide roll compensation as follows:
            %
            \begin{equation}
            \begin{split}
            % F_{B} = R_{BL} * F_L\\
            \roll\refer &= atan2(F_{B}(1), \sqrt{F_{B}(0)^2,F_{B}(2)^2})\\
            F_{B}(1) &= 0\\
            R_{\roll\refer} &= 
            \begin{bmatrix}
                1 & 0 & 0\\
                0 & cos(\roll\refer) & -sin(\roll\refer)\\
                0 & sin(\roll\refer) & cos(\roll\refer)
            \end{bmatrix}\\
            R_{WB} &*= R_{\roll\refer}
            \end{split} \label{eq4}
            \end{equation}
             %
            Where $\roll\refer \in \nR{}$ is represents the roll angle reference, $F_{B} \in \nR{3}$ the desired command force vector in body frame, $\rotMatWB \in \nR{3 \times 3}$ the rotation matrix from body to world frame\\
            %
            For what concern the attitude and rates control errors:
            %
            \begin{equation}
            \label{eq5}
            \begin{split}
            \angErrorL &= \frac{1}{2} \rotMatLB \left[ \rotMatWB\transpose \rotMatWB\refer - \rotMatWB\refer{}\transpose \rotMatWB \right]^\vee, \\
            \L\angVel\refer &= \kpAng\angErrorL,\\
            %+ \begin{bmatrix} 0 \\ 0 \\ yaw_{sp} \end{bmatrix} \\
            \angVelErrorL &= \L\angVel\refer - \rotMatLB\angVel,\\
            \angCumulativeErrorL &= \kpRate \angVelErrorL + \kiRate \int_0^t\angVelErrorL - \kdRate \angAcc, \\
            twist_{B} &= \angVelErrorB x (I * \angVelErrorB), \\
            omega &= \angVelErrorB x (R_{LB} * \angCumulativeErrorL), \\
            desiredAccel_{ang, L} &= \angCumulativeErrorL + R_{LB} * (I*twist_{B} - omega), \\
            M_{L} &= I*desiredAccel_{ang, L},
            \end{split}
            \end{equation}
            %
            where $\angErrorL \in \nR{3}$ is the attitude error, $\L\angVel\refer$ the angular rate reference,
            %$k_{p, att}$ the attitude gain for the P part of the controller, $yaw_{sp}$ the yaw setpoint,
            $\angVelErrorL$ the rate error in the L frame, $\angVel$ the angular rate, $\angCumulativeErrorL$ the total angular error, $\kpAng$, $\kpRate$, $\kiRate$, $\kdRate \in \nR{3\times3}$ are positive definite diagonal gain matrices.
            $twist_{B} \in \nR{3}$ is the current twist in the body frame, $\angVelErrorB \in \nR{3}$ is the angular velocity error in the body frame, $desiredAccel_{ang, L} \in \nR{3}$ is the desired angular acceleration, $I \in \nR{3 \times 3}$ is the inertia matrix, $M_L \in \nR{3}$ is the desired moment vector with all the components in all three directions.
            The angular error in L frame is used to calculate the desired angular acceleration also in L frame, then the desired torque vector in L frame can be calculated. \\
            %
          A low-level controller is implemented inside the Pixhawk and utilizes cascaded PID gains to control both position and attitude, which, roll excluded are decoupled. The controller receives data from odometry sensors, and inputs in form of setpoints, and it uses these information to calculate the desired wrench vector. \\
          %The presented MAV can flight in manual mode with a normal radio transmitter or in offboard mode by sending commands from a base station. In manual mode, the controller will take the setpoints from the input given by the sticks of the radio and there will be no position control since the platform has no information about the current position, there will still be control on velocity and attitude with the data provided by the IMU of the Pixhawk.
          %The Raspberry Pi is used as an onboard computer and, with the help of Vicon cameras that recognizes special markers placed on the frame of the drone, it is possible to have position control as well in addition to velocity and attitude control. The desired setpoints in Vicon coordinates are sent to the drone through the onboard computer and the data on actual position comes from the Vicon system, with this information the Pixhawk, at each time step, will calculate the desired wrench vector to adjust position and orientation, and then by solving the system of equations \ref{eq1} the needed actuator signals. \\
          The controller takes informations about velocity, attitude and rates from the IMU of the Pixhawk and, if present, position from the Vicon system. First the position controller will calculate the forces of the wrench vector needed to try to reach the desired setpoint, received either from the remote control nor computer. After calculating the forces, if there if any desired force in \textit{y}-direction the roll angle will be calculated and the attitude setpoint for roll adjusted consequently. Finally, the adjusted attitude setpoint is fed to a cascade PID controller, the first attitude P controller compares it with the measured attitude and the resulting rate is passed into the rates PID controller, which also takes in the rates from IMU sensors. At this point the allocation system receives the desired wrench vector, composed by the calculated desired forces and torques, and the needed actuator signals are found and passed to the motors and servomotors.
          
          \item Actuator allocation. \\
          %Instead of having an allocation matrix with the contribution of each motor in any direction to calculate the correct angles and motor rotational speeds, the general system of equations for forces and torques is used. The PX4 code inside the Pixhawk will solve, at each time step, the system of equations \ref{eq1} and calculate the desired motor thrusts and servo angles to achieve the desired wrench vector.
          The actuators allocation is given by the equations
          \begin{figure}
              \centering
              \includegraphics[width=1\columnwidth]{convention.png}
              \caption{Convention for the Mini Voliro}
              \label{pics:convention}
          \end{figure}
          \begin{equation} \label{eq1}
              \begin{split}
                  F_{x} & = T_{12}\sin\alpha_{1} - T_{34}\sin\alpha_{0}\\
                  F_{y} & = 0 \\
                  F_{z} & = - T_{12}\cos\alpha_{1} - T_{34}\cos\alpha_{0} - T_{5} \\
                  M_{x} & = l_{1}(T_{12}\cos\alpha_{1} - T_{34}\cos\alpha_{0}) \\
                  M_{y} & = -l_{2}T_{5}\\
                  M_{z} & = l_{1}(+T_{12}\sin\alpha_{1} + T_{34}\sin\alpha_{0}) - k_{d}T_{5} ,
              \end{split}
          \end{equation}
          here $l_{1}$ is the distance from the center of the motor of one arm to the center of the frame, $l_{2}$ the distance from the center of the tail motor to the center of the frame, T are the thrusts produced by the respective motors, and $\alpha$ are the angles of the servomotors.
          %
          These equation can be rewritten as
          %The moment produced by the thrust coefficient $k_{d}$ of the rear motor, multiplied with the thrust of the rear motor, is ignored into the allocation since it can be easily be handled by the controller. \\
          \begin{equation}
              \begin{bmatrix}
                  F_{x}\\
                  F_{z}\\
                  M_{x}\\
                  M_{y}\\
                  M_{z}
              \end{bmatrix} =
              \begin{bmatrix}
                  1 & 0 & -1 & 0 & 0\\
                  0 & -1 & 0 & -1 & -1\\
                  0 & l_1 & 0 & -l_1 & 0\\
                  0 & 0 & 0 & 0 & -l_2\\
                  l_1 & 0 & l_1 & 0 & -k_d\\
              \end{bmatrix}
              \inputSin , 
              \label{allocation}
          \end{equation}
          with the vector $\inputSin \in \nR{5}$
          \begin{equation}
              \inputSin = 
              \begin{bmatrix}
                  T_{12}sin(\alpha_1)\\
                  T_{12}cos(\alpha_1)\\
                  T_{34}sin(\alpha_0)\\
                  T_{34}cos(\alpha_0)\\
                  T_5
              \end{bmatrix} .
          \end{equation}
          From \eqref{allocation}, the thrust commands and the tilt angles can be found as
          \begin{equation}
            \begin{split}
            T_{12} &= \sqrt{u_1^2 + u_2^2}\\
            T_{34} &= \sqrt{u_3^2 + u_4^2}\\
            \alpha_0 &= \text{atan2}(u_1,u_2)\\
            \alpha_1 &= \text{atan2}(u_3,u_4) .\\
            \end{split}
            \label{thrusts_tilts}
            \end{equation}
          From there the rotational speeds of the motors can be calculated by knowing the motor coefficient $k_{f}$ and assuming a quadratic relationship.
          \begin{equation}
              \begin{split}
                  \omega_{1} & = \omega_{2} = \sqrt{\dfrac{T_{12}}{2k_{f}}}\\
                  \omega_{3} & = \omega_{4} = \sqrt{\dfrac{T_{34}}{2k_{f}}}\\
                  \omega_{5} & = \text{sign}(T_5)\sqrt{\dfrac{\norm{T_{5}}}{k_{f, rear}}}
              \end{split}
              \label{motor_relation}
          \end{equation}
          Since the rear motor is bidirectional, the sign of the desired rear trust $T_5$ must be specifically taken into account in \eqref{motor_relation}.
        %   For negative $T_{5}$, when the rear motor is spinning in opposite direction, a minus sign is inserted in the code to calculate the omega avoiding negative values under the square root.
        %   Rotational speeds and servo angles are then scaled into signals with values between -1 and 1 and passed through the mixer to the actuators.


\end{itemize}




%%%%%%NOTES
Then we can define the translational and rotational dynamics of the \ac{MAV} as
\begin{subequations}
    \label{drone_model}
    \begin{IEEEeqnarray} {ll}
        \mass\left(\W{\acc}+\rotMatWB\B{\angVel}\times\B{\vel}\right) = \W\gravityForce + \W\forceCommand\\
        \inertia\B\angAcc + \B\angVel\times \inertia\B{\angVel} = \torqueCommand,
    \end{IEEEeqnarray}
\end{subequations}
where $\mass \in \nR{}$ is the total mass of the platform, $\inertia \in \nR{3\times3}$ is the inertia matrix in $\frameB$, $\gravityForce \in \nR{3}$ is the gravity force vector, $\angVel \in \nR{3}$ is the platform's angular velocity, and $\forceCommand \in \nR{3}$ and $\torqueCommand \in \nR{3}$ are the force and torque commands, respectively.
%
Because the system cannot produce instantaneous thrust along its body $\B\y$ axis, a hierarchical controller between position and attitude is necessary.
%
The control hierarchy still addresses the full actuation in the pitching dynamics.
%

Consider the position and velocity errors of the translational dynamics as
\begin{subequations}
    \label{eq:pos_errors}
    \begin{IEEEeqnarray} {ll}
        \W\positionError &=  \W\pos\refer - \W\pos,\\
        \W\velocityError &= \W\vel\refer - \rotMatWB\B\vel,
    \end{IEEEeqnarray}
\end{subequations}
where $\positionError \in \nR{3}$ and $\velocityError \in \nR{3}$ are the position and velocity errors, respectively, and the quantities $(\cdot)\refer$ come instead from a suitable trajectory planner.
%
%From \eqref{pos_errors} the force control vector $\forceCommand \in \nR{3}$ can be computed as
Based on \eqref{eq:pos_errors} we define the Proportional-Derivative (PD) control law as
\begin{equation}
\begin{split}
    \W\forceCommand =& \kpPos \W\positionError + \kdPos \W\velocityError - \W\gravityForce +\\&+ \mass \left(\W\acc\refer+\rotMatWB\B{\angVel}\times\B{\vel}\right),    
\end{split}
\end{equation}
%
from which we obtain $\B\forceCommand = \rotMatWB\transpose \W\forceCommand$.
%
Note that $\B\forceCommand$ is a vector in $\nR{3}$, but the platform cannot exert forces in the ${}_B\vec{y}$ body axis.
%
For this reason, we consider a new command vector $\B\underForceCommand = \left[ 0 \vSpace \B{}\forceCommandi{1} \vSpace \B{}\forceCommandi{2} \right]\transpose$, from which the commanded force along $\B x$ has been removed, since the platform can exert it instantaneously and it does not need to be a reference for the attitude controller.
%
We compute the desired force direction vector from the position loop as $\B{\vec{z}}\des = \frac{\B\underForceCommand}{\norm{\B\underForceCommand}}$.
